On the Curse of Memory in Recurrent Neural Networks: Approximation and Optimization Analysis

We study the approximation properties and optimization dynamics of recurrent neural networks (RNNs) when applied to learn input-output relationships in temporal data. We consider the simple but representative setting of using continuous-time linear RNNs to learn from data generated by linear relationships. Mathematically, the latter can be understood as a sequence of linear functionals. We prove a universal approximation theorem of such linear functionals, and characterize the approximation rate and its relation with memory. Moreover, we perform a fine-grained dynamical analysis of training linear RNNs, which further reveal the intricate interactions between memory and learning. A unifying theme uncovered is the non-trivial effect of memory, a notion that can be made precise in our framework, on approximation and optimization: when there is long term memory in the target, it takes a large number of neurons to approximate it. Moreover, the training process will suffer from slow downs. In particular, both of these effects become exponentially more pronounced with memory - a phenomenon we call the "curse of memory". These analyses represent a basic step towards a concrete mathematical understanding of new phenomenon that may arise in learning temporal relationships using recurrent architectures.

==> algorithm.tex <==
% \section{Numerical Experiments}

% \QL{Maybe no need for arxiv version?}
% \JH{Or even no need for ICLR paper?}


==> asymptotics.tex <==
\subsection{Asymptotic Analysis of Plateauing}

For simplicity, we still only consider the diagonal case, but a simpler setup. Set the hypothesis space
\begin{align}
\hat{\rho}(t ; w) := \sum_{j=1}^{m}e^{-w_j t},\quad w_j>0,
\end{align}
and the ground truth
\begin{align}
\rho(t) := \sum_{j=1}^{m^*}e^{-w^*_j t},
\end{align}
where $w_j^*>0$ and $w_i^*\ne w_j^*$ for any $i\ne j$. To obtain a clean form, consider the loss with infinite time horizon
\begin{align}
J_\infty(w) = \int_{0}^{\infty} (\hat{\rho}(t; w) - \rho(t))^2 dt.
\end{align}
In the following, we will always set $m\ge m^*=2$.


\subsubsection{2-dimensional case}

\textbf{(1)~Setup}

For $m=2$, consider the 2-parameter optimization problem
\begin{align}\label{2wInftyOpt}
\min_{w_1,w_2>0}J_\infty(w_1,w_2):=\int_{0}^{\infty}\left[(e^{-w_1t}+e^{-w_2t})-(e^{-w_1^*t}+e^{-w_2^*t})\right]^2dt,
\end{align}
where $w_1^*,w_2^*>0$ and $w_1^*\ne w_2^*$. Obviously $(w_1^*,w_2^*)$ and $(w_2^*,w_1^*)$ are two different global minimizers. A direct computation shows
\begin{align}\label{2wInftyLoss}
\begin{split}
J_{\infty}(w_1,w_2)&=\left(\frac{1}{2w_1}+\frac{1}{2w_2}+\frac{2}{w_1+w_2}-\frac{2}{w_1+w_1^*}-\frac{2}{w_2+w_2^*}-\frac{2}{w_1+w_2^*}-\frac{2}{w_2+w_1^*}\right)\\
&\quad +\left(\frac{1}{2w_1^*}+\frac{1}{2w_2^*}+\frac{2}{w_1^*+w_2^*}\right),
\end{split}
\end{align}
and
\begin{equation}\label{2wInftyGrad}
\left\{
\begin{array}{lr}
\frac{\partial J_{\infty}}{\partial w_1}=-\frac{1}{2w_1^2}+\frac{2}{(w_1+w_1^*)^2}-\frac{2}{(w_1+w_2)^2}+\frac{2}{(w_1+w_2^*)^2}, &  \\
\frac{\partial J_{\infty}}{\partial w_2}=-\frac{1}{2w_2^2}+\frac{2}{(w_2+w_1^*)^2}-\frac{2}{(w_1+w_2)^2}+\frac{2}{(w_2+w_2^*)^2}.&  
\end{array}
\right.
\end{equation}
The aim is to investigate the gradient flow of $J_{\infty}(w_1,w_2)$: 
\begin{align}\label{2wInftyGradFlow}
\left\{
\begin{array}{lr}
w_1'(\tau)=\frac{1}{2w_1^2(\tau)}-\frac{2}{(w_1(\tau)+w_1^*)^2}+\frac{2}{(w_1(\tau)+w_2(\tau))^2}-\frac{2}{(w_1(\tau)+w_2^*)^2}, &  \\ w_2'(\tau)=\frac{1}{2w_2^2(\tau)}-\frac{2}{(w_2(\tau)+w_1^*)^2}+\frac{2}{(w_1(\tau)+w_2(\tau))^2}-\frac{2}{(w_2(\tau)+w_2^*)^2},&  
\end{array}
\right.
\end{align}
with some initial value $w_1(0),w_2(0)>0$. Denote $\bw_0:=(w_1(0),w_2(0))$. Obviously, the nonlinear system (\ref{2wInftyGradFlow}) does not have an analytic solution, but we want to analyze the convergence property of $(w_1(\tau),w_2(\tau))$ as $\tau\to+\infty$ under different $\bw_0$'s.

\textbf{Symmetry argument}. $\nabla J_{\infty}(w_1,w_2)$, or dynamical system (\ref{2wInftyGradFlow}) is symmetric between $w_1$ and $w_2$, leading to the fact that:
\begin{itemize}
	\item $\nabla J_{\infty}(w_1,w_2)=0$ implies $\nabla J_{\infty}(w_2,w_1)=0$;
	\item For any $\tau_0\ge 0$, $w_1(\tau_0)=w_2(\tau_0)$ implies $w_1'(\tau_0)=w_2'(\tau_0)$, hence $w_1(\tau)=w_2(\tau)$ for any $\tau\ge \tau_0$. That is to say, $w_1(0)=w_2(0)$ implies $w_1(\tau)=w_2(\tau)$ for any $\tau\ge 0$. Under this type of initialization, for $i=1,2$, $w_i(\tau)$ satisfies the one-dimensional ODE
	\begin{align} \label{1D-ODE}
	v'(\tau)&=\frac{1}{v^2(\tau)}-\frac{2}{(v(\tau)+w_1^*)^2}-\frac{2}{(v(\tau)+w_2^*)^2}.
	\end{align}
\end{itemize}

\textbf{(2)~Numerical examples}

Some numerical tests are performed on (\ref{2wInftyGradFlow}) to obtain illustrations. For convenience, for $i=1,2$, we assume that $w_i^*=O(1)$, $w_i(0)=o(1)$, and $w_1^*<w_2^*$, $|w_1(0)-w_2(0)|\ll 1$. By (\ref{2wInftyOpt}) or (\ref{2wInftyLoss}), the same scaling process can be done on $w_i$ and $w_i^*$ simultaneously, only causing a scaling factor on $J_\infty(\cdot)$. Therefore, initializing $w_i$ in a small interval for generical $w_i^*$'s is equivalent to generically initializing $w_i$ for large $w_i^*$'s. We utilize  Adams-Bashforth-Moulton method to numerically solve (\ref{2wInftyGradFlow}). Fig. 1 shows the separation of parameters and plateauing of the loss under two different initializations: $w_1(0)=w_2(0)=\xi$ and $w_1(0)=\xi$, $w_2(0)=\xi+\delta$. Here $0<\delta<\xi\ll 1$, and $\delta$, $\xi$ has the same magnitude. 

\begin{figure}[htb!]
	\centering
	\includegraphics[height=6.5cm,width=8.95cm]{figures/ParaDeltaRand.png}
	\includegraphics[height=6.5cm,width=8.95cm]{figures/LossDeltaRand.png}
	\caption{The separation of parameters and plateauing of the loss under two initializations: $\bw_0=(\xi,\xi)$ and $\bw_0^{\delta}=(\xi,\xi+\delta)$. Here $\delta=10^{-4}$, $\xi=\delta\xi_0$, where $\xi_0\sim\mathcal{U}[1,10)$, and $w_i^*\sim\mathcal{U}[1,10)$.}
\end{figure}

By Fig. 1, the dynamics of (\ref{2wInftyGradFlow}) with the initial value $\bw_0^\delta$ can be understood as follows: 
\begin{itemize}
	\item Stage 1: the convergence process of the one-dimensional ODE (\ref{1D-ODE}). The convergence of (\ref{1D-ODE}) as $\tau\to+\infty$ will be verified later (see Lemma \ref{lmm:1D-ODEConverge});
	\item Stage 2: the convergence state of (\ref{1D-ODE}). This leads to the plateauing of the loss $J_\infty(\cdot)$;
	\item Stage 3: the separation of parameters. This leads to the loss decreases again, and the dynamical system (\ref{2wInftyGradFlow}) finally converges. 
\end{itemize}
Next, some asymptotic analysis is performed to quantify the timescales of plateauing with respect to $\delta$.


\textbf{(3)~Asymptotic analysis}

\begin{lemma}\label{lmm:1D-ODEConverge}
	For the one-dimensional ODE (\ref{1D-ODE}) with $v(0)>0$, $v(\tau)$ converges as $\tau\to+\infty$.
\end{lemma}

\begin{proof}
(\ref{1D-ODE}) can be written as
\begin{align}\label{1D-ODEp}
v'(\tau)=\frac{p(v(\tau))}{v^2(\tau)(v(\tau)+w_1^*)^2(v(\tau)+w_2^*)^2},
\end{align}
where $p(v):=(v+w_1^*)^2(v+w_2^*)^2-2v^2\left[(v+w_1^*)^2+(v+w_2^*)^2\right]$ is a fourth-order polynomial. Since 
$$p(w_1^*)=2w_1^{*2}(3w_1^*+w_2^*)(w_2^*-w_1^*)>0,\quad p(w_2^*)=2w_2^{*2}(3w_2^*+w_1^*)(w_1^*-w_2^*)<0,$$
there exists $c\in (w_1^*,w_2^*)$ such that $p(c)=0$ and $p(v)$ changes the sign at $v=c$. Let $0<c_1<\cdots<c_k<+\infty$ be the positive roots of $p(v)$, and $p(v)$ changes the sign at $v=c_j$, $j=1,2\cdots,k$, then $1\le k\le 4$. Hence, $p(v)$ has the following decomposition: 
$$p(v)=(v-c_1)\cdots(v-c_k)\cdot q(v),\quad v\in(0,+\infty),$$
where $q(v)<0$ for any $v>0$\footnote{Obviously $q(v)$ does not change the sign on $(0,+\infty)$, since $q(v)$ contains all the negative and complex roots of $p(v)$, also all the positive roots at which $p(v)$ does not change the sign. As $p(+\infty)=-\infty$, we have $q(v)<0$.}. Then (\ref{1D-ODEp}) becomes
\begin{align}\label{1D-ODEpDec}
v'(\tau)=(v(\tau)-c_1)\cdots(v(\tau)-c_k)\cdot\frac{q(v(\tau))}{v^2(\tau)(v(\tau)+w_1^*)^2(v(\tau)+w_2^*)^2},
\end{align}
or
\begin{align*}
\frac{1}{(v(\tau)-c_1)\cdots(v(\tau)-c_k)}\frac{v^2(\tau)(v(\tau)+w_1^*)^2(v(\tau)+w_2^*)^2}{q(v(\tau))}dv(\tau)=d\tau.
\end{align*}
Integrating from $0$ to $t$, we have
\begin{align}\label{1D-ODEInt}
t&=\int_0^t\frac{1}{(v(\tau)-c_1)\cdots(v(\tau)-c_k)}\frac{v^2(\tau)(v(\tau)+w_1^*)^2(v(\tau)+w_2^*)^2}{q(v(\tau))}dv(\tau)\nonumber\\
&=\int_{v(0)}^{v(t)}\frac{1}{(v-c_1)\cdots(v-c_k)}\frac{v^2(v+w_1^*)^2(v+w_2^*)^2}{q(v)}dv.
\end{align}
Let $\mathcal{I}_j:=[c_{j},c_{j+1})$, $j=1,2,\cdots,k-1$, and $\mathcal{I}_0:=(0,c_{1})$, $\mathcal{I}_k:=[c_{k},+\infty)$, then $v(0)\in\cup_{j=0}^{k}\mathcal{I}_j$. We have the following discussion:
\begin{itemize}
	\item $v(0)\in\mathcal{I}_j$, $j=1,2,\cdots,k-1$: if $v(0)=c_j$, then $v(\tau)=c_j$; if $v(0)\in (c_{j},c_{j+1})$, then $v(\tau)$ is monotonous if $v(\tau)\in (c_{j},c_{j+1})$ according to (\ref{1D-ODEpDec});
	\item $v(0)\in\mathcal{I}_0$: notice that $p(0)=(w_1^*w_2^*)^2>0$, then $k$ is odd, and $v(\tau)$ is monotonously increasing if $v(\tau)\in (0,c_{1})$ according to (\ref{1D-ODEpDec});
	\item $v(0)\in\mathcal{I}_k$: if $v(0)=c_k$, then $v(\tau)=c_k$; if $v(0)>c_k$, notice that $p(v)<0$ for any $v>c_k$, we have that $v(\tau)$ is monotonously decreasing if $v(\tau)\in (c_{k},+\infty)$ according to (\ref{1D-ODEp}).
\end{itemize}
Let $c_0=0$, $c_{k+1}=+\infty$. For $j=0,1,\cdots,k$, assume $v(0)\in (c_{j},c_{j+1})$, then we have $v(\tau)\in [c_{j},c_{j+1}]$, hence $v(\tau)$ is monotonous for any $\tau\ge 0$. As a result, $v(+\infty)$ exists. Taking $t\to+\infty$ in (\ref{1D-ODEInt}), we obtain
\begin{align}\label{1D-ODEIntLim}
\int_{v(0)}^{v(+\infty)}\frac{1}{(v-c_1)\cdots(v-c_k)}\frac{v^2(v+w_1^*)^2(v+w_2^*)^2}{q(v)}dv=+\infty.
\end{align}
This implies $v(+\infty)=c_j$ or $v(+\infty)=c_{j+1}$. That is to say, when $\tau\to+\infty$, $v(\tau)$ converges to one of the positive roots of $p(v)$.
\end{proof}

\begin{proposition}\label{prop:2D-ODEPlateau}
	For a sufficiently long time of separation or plateauing (typically corresponding to a sufficiently small $\delta$), the timescales of plateauing is $\Theta(\ln(1/\delta))$.
\end{proposition}

\begin{proof}
\textbf{(i)~Separation of parameters}.~For any $\epsilon>0$, $\epsilon\ll 1$, write
\begin{align}\label{AsyExpan}
w_i(\tau)=w(\tau)+\epsilon\cdot v_i(\tau)+O(\epsilon^2), \quad i=1,2.
\end{align}
Then for any $c>0$, 
\begin{align}\label{AsyExpan1}
\frac{1}{(w_i(\tau)+c)^2}&=\frac{1}{[(w(\tau)+c)+\epsilon\cdot v_i(\tau)+O(\epsilon^2)]^2}
=\frac{1}{(w(\tau)+c)^2+\epsilon\cdot 2v_i(\tau)(w(\tau)+c)+O(\epsilon^2)}\nonumber\\
&=\frac{1}{(w(\tau)+c)^2}\frac{1}{1+\epsilon\cdot 2v_i(\tau)/(w(\tau)+c)+O(\epsilon^2)}\nonumber\\
&=\frac{1}{(w(\tau)+c)^2}\left(1-\epsilon\cdot \frac{2v_i(\tau)}{w(\tau)+c}+O(\epsilon^2)\right)\nonumber\\
&=\frac{1}{(w(\tau)+c)^2}-\epsilon\cdot \frac{2v_i(\tau)}{(w(\tau)+c)^3}+O(\epsilon^2),
\end{align}
where we use the fact that $w_i(\tau)>0$ for any $\tau\ge 0$
\footnote{By (\ref{2wInftyGradFlow}), we have $w'_i(\tau)\to +\infty$ if $w_i(\tau)\to 0^+$. Hence $w_i(\tau)>0$ for any $\tau\ge 0$ as long as $w_i(0)>0$. By (\ref{AsyExpan}), on any finite interval $[0,T_0]$, we have $w(\tau)\ge \frac{1}{2}\min\limits_{\tau\in[0,T_0]}w_1(\tau)>0$.}. 
Similarly, 
\begin{align}\label{AsyExpan2}
\frac{1}{(w_1(\tau)+w_2(\tau))^2}=\frac{1}{4w^2(\tau)}-\epsilon\cdot \frac{v_1(\tau)+v_2(\tau)}{4w^3(\tau)}+O(\epsilon^2).
\end{align}
Substituting $w_i(\tau)$ in (\ref{2wInftyGradFlow}) by (\ref{AsyExpan}), (\ref{AsyExpan1}) and (\ref{AsyExpan2}), we obtain
\begin{align}
w'(\tau)&=\frac{1}{w^2(\tau)}-\frac{2}{(w(\tau)+w_1^*)^2}-\frac{2}{(w(\tau)+w_2^*)^2},\quad\mathrm{at~}O(1)~\mathrm{level}, \label{O1Level}\\
v_i'(\tau)&=-\frac{v_i(\tau)}{w^3(\tau)}+\frac{4v_i(\tau)}{(w(\tau)+w_1^*)^3}+\frac{4v_i(\tau)}{(w(\tau)+w_2^*)^3}-\frac{v_1(\tau)+v_2(\tau)}{2w^3(\tau)},\quad\mathrm{at~}O(\epsilon)~\mathrm{level}. \label{OepsLevel}
\end{align}
Denote $\Delta(\tau):=v_2(\tau)-v_1(\tau)$, $\tau\ge 0$. By (\ref{OepsLevel}), 
\begin{align}\label{DltODE}
\Delta'(\tau)=-\frac{\Delta(\tau)}{w^3(\tau)}+\frac{4\Delta(\tau)}{(w(\tau)+w_1^*)^3}+\frac{4\Delta(\tau)}{(w(\tau)+w_2^*)^3}:=\Delta(\tau)W(w(\tau)),
\end{align}
where $W(w):=-\frac{1}{w^3}+\frac{4}{(w+w_1^*)^3}+\frac{4}{(w+w_2^*)^3}$, $w>0$. By Footnote 2, $w(\tau)>0$, hence $W(w(\tau))$ is well defined. Solving (\ref{DltODE}) gives
\begin{align}\label{Dlt}
\Delta(\tau)=\Delta(0)\exp\left(\int_0^\tau W(w(s))ds\right).
\end{align} 
Therefore, combining with (\ref{AsyExpan}), we have the separation gap 
\begin{align}\label{SepParaGap}
|w_2(\tau)-w_1(\tau)|=\epsilon|\Delta(\tau)|+O(\epsilon^2)\stackrel{(a)}{=}\delta\exp\left(\int_0^\tau W(w(s))ds\right)+O(\epsilon^2),
\end{align} 
where $(a)$ is due to $\delta=|w_2(0)-w_1(0)|=\epsilon|\Delta(0)|+O(\epsilon^2)$, and $W(w(\tau))=O(1)$ on any finite interval. 

To obtain a separation tolerance $|w_2(\tau)-w_1(\tau)|\ge\epsilon_1\ge c\delta$, where $c>1$ in general, we have to require $\delta\exp\left(\int_0^\tau W(w(s))ds\right)\ge\epsilon_1$, i.e. 
\begin{align*}
\int_0^\tau W(w(s))ds\ge\ln(\epsilon_1/\delta)\ge \ln c>0.
\end{align*} 
We will show the integral $\int_0^\tau W(w(s))ds$ is (almost) linear in $\tau$ (for a sufficiently large timescale of separation). In fact, according to Lemma \ref{lmm:1D-ODEConverge}, $w(+\infty)$ exists. Fix $\epsilon_0>0$, $\epsilon_0\ll 1$, and define 
\begin{align}\label{Treach}
T_{\mathrm{reach}}:=\inf\{\tau:|w(s)-w(+\infty)|\le \epsilon_0,~\forall s\ge \tau\}.
\end{align} 
For a sufficiently large timescale of separation, typically $T_{\mathrm{separation}}\gg T_{\mathrm{reach}}$, we have 
\begin{align*}
0<\ln c\le\ln(\epsilon_1/\delta)
&\le \int_0^{T_{\mathrm{reach}}}W(w(s))ds
+\int_{T_{\mathrm{reach}}}^{T_{\mathrm{separation}}} W(w(s))ds\\
&\approx W(w(s_0))\cdot T_{\mathrm{reach}}+ W(w(+\infty))\cdot(T_{\mathrm{separation}}-T_{\mathrm{reach}}),\quad (0<s_0<T_{\mathrm{reach}})
\end{align*} 
and certainly $W(w(+\infty))>0$. This implies
\begin{align}\label{TSep}
T_{\mathrm{separation}}\approx\frac{\ln(1/\delta)}{W(w(+\infty))}+\left[T_{\mathrm{reach}}+\frac{\ln{\epsilon_1}-W(w(s_0)) T_{\mathrm{reach}}}{W(w(+\infty))}\right],
\end{align} 
or $T_{\mathrm{separation}}=\Theta(\ln(1/\delta))$.

\textbf{(ii)~Plateauing of the loss}.~Now we turn to the loss (\ref{2wInftyLoss}). Under the variable transform 
\begin{align*}
u_1=\frac{w_1+w_2}{2},\quad u_2=\frac{w_1-w_2}{2},
\end{align*} 
or the inverse 
\begin{align*}
w_1=u_1+u_2,\quad w_2=u_1-u_2,
\end{align*} 
the loss function (\ref{2wInftyLoss}) can be transformed as
\begin{align}\label{2wInftyLossTrans}
\begin{split}
\tilde{J}(u_1,u_2)&=\frac{1}{2}\left(\frac{1}{u_1+u_2}+\frac{1}{u_1-u_2}\right)
-2\left(\frac{1}{u_1+u_2+w_1^*}+\frac{1}{u_1-u_2+w_1^*}\right)
\\&\quad -2\left(\frac{1}{u_1+u_2+w_2^*}+\frac{1}{u_1-u_2+w_2^*}\right)
+\frac{1}{u_1}+c^*,
\end{split}
\end{align}
where $c^*=\frac{1}{2w_1^*}+\frac{1}{2w_2^*}+\frac{2}{w_1^*+w_2^*}$. In the plateauing, $u_1(\tau)=\Theta(1)$, and $u_2(\tau)=O(\epsilon)$ by (\ref{SepParaGap}). For any $u_1>0$, $u_1=\Theta(1)$, define $J_{u_1}(u_2):=\tilde{J}(u_1,u_2)$. We can utilize the Taylor expansion to estimate $|J_{u_1}(u_2)-J_{u_1}(0)|$ for $|u_2|\ll 1$, where $J_{u_1}(0)=\tilde{J}(u_1,0)=J_\infty(w_1,w_2)|_{w_1=w_2}$.

For any $c>0$, we have
\begin{align}\label{TayExp+}
\frac{1}{u_1+u_2+c}-\frac{1}{u_1+c}
&=\frac{1}{u_1+c}\left(\frac{1}{1+\frac{u_2}{u_1+c}}-1\right)\nonumber\\
&=\frac{1}{u_1+c}\left(1-\frac{u_2}{u_1+c}+\frac{u_2^2}{(u_1+c)^2}+O(u_2^3)-1\right)\nonumber\\
&=-\frac{u_2}{(u_1+c)^2}+\frac{u_2^2}{(u_1+c)^3}+O(u_2^3).
\end{align} 
Similarly,
\begin{align}\label{TayExp-}
\frac{1}{u_1-u_2+c}-\frac{1}{u_1+c}
=\frac{u_2}{(u_1+c)^2}+\frac{u_2^2}{(u_1+c)^3}+O(u_2^3).
\end{align} 
Substituting the corresponding terms in (\ref{2wInftyLossTrans}) with (\ref{TayExp+}) and (\ref{TayExp-}), we obtain 
\begin{align}\label{TayExpLoss}
\tilde{J}(u_1,u_2)-\tilde{J}(u_1,0)=
\frac{u_2^2}{u_1^3}-\frac{4u_2^2}{(u_1+w_1^*)^3}-\frac{4u_2^2}{(u_1+w_2^*)^3}+O(u_2^3),
\end{align} 
i.e.
\begin{align}\label{PlaLossGap}
|J_\infty(w_1,w_2)-J_\infty(w,w)|=|\tilde{J}(u_1,u_2)-\tilde{J}(u_1,0)|
=O(u_2^2)=O((w_1-w_2)^2).
\end{align} 
By (\ref{SepParaGap}), 
\begin{align*}
(w_2(\tau)-w_1(\tau))^2=\delta^2\exp\left(2\int_0^\tau W(w(s))ds\right)+O(\epsilon^2).
\end{align*} 
Therefore, to obtain a plateauing-escaping tolerance $|J_\infty(w_1(\tau),w_2(\tau))-J_\infty(w(\tau),w(\tau))|\ge \epsilon_2$, the following analysis is totally the same as \textbf{(i)}, except for replacing $\delta$ by $\delta^2$, and $W(w)$ by $2W(w)$. According to (\ref{TSep}),  
\begin{align}\label{TPla}
T_{\mathrm{plateauing}}\approx\frac{\ln(1/\delta)}{W(w(+\infty))}+\left[T_{\mathrm{reach}}+\frac{\ln{\epsilon'_2}-2W(w(s_0)) T_{\mathrm{reach}}}{2W(w(+\infty))}\right],
\end{align} 
where $\epsilon'_2$ is proportional to $\epsilon_2$. That is to say, $T_{\mathrm{plateauing}}=\Theta(\ln(1/\delta))$.
\end{proof}

\subsubsection{Multi-dimensional case}
\hl{To be completed}


==> experiments.tex <==
\section{Experiments}

Here, we will conduct a sequence of experiments to study the dynamics of learning functionals $H_t$. We will consider the following parameterizations of $H_t$

\begin{enumerate}
    \item Langevin dynamics: $\bs{x}_{0:t} \mapsto y_t$ as
    \begin{align}
        \dot{q}_{t} &= p_{t} & &q_0 = 0\\
        \dot{p}_{t} &= - \nabla U(q_{t}) - \gamma p_{t} + \sqrt{ \frac{2\gamma}{\beta}} x_{t} & &p_0 = 0 \\
        y_{t} &= q_t
    \end{align}
    \item Generalized Langevin dynamics: $\bs{x}_{0:t} \mapsto y_t$ as
    \begin{align}
        \dot{q}_{t} &= p_{t} & &q_0 = 0\\
        \dot{p}_{t} &= - \nabla U(q_{t}) - \gamma p_{t}
        - \int_{0}^{t} K(s, t) p_{s} ds
        + \sqrt{ \frac{2\gamma}{\beta}} x_{t} & &p_0 = 0\\
        y_{t} &= q_t
    \end{align}
    Here, memory is also incorporated explicitly in the equations.
    We can consider the following kernels:
    \begin{itemize}
        \item Exponential: $K(s, t) = e^{- c |s - t|}$
        \item Power law: $K(s, t) = \frac{1}{1 + c|s - t|}$
        \item Sine: $K(s, t) = \sin(c|s-t|)$
    \end{itemize}
\end{enumerate}

For all the subsequent experiments, we will consider the potential $U(x) = \| x \|^2 / 2$ so that $H_t$ is always a linear functional.

\newpage
\subsection{Initialization}

To test how initialization affects learning dynamics, we vary the initialization of the recurrent kernels $U_h$ and test RNN and GRU performance on learning Langevin dynamics. The results are shown in Fig.~\cref{fig:init_adam} (Adam optimizer) and Fig.~\cref{fig:init_sgd}
\begin{figure}[htb!]
    \centering
    \includegraphics[width=\textwidth]{figures/initialization_adam}
    \caption{Initialization study using adam optimizer.}
    \label{fig:init_adam}
\end{figure}
\begin{figure}[htb!]
    \centering
    \includegraphics[width=\textwidth]{figures/initialization_sgd}
    \caption{Initialization study using SGD optimizer.}
    \label{fig:init_sgd}
\end{figure}


\newpage
\subsection{Memory and Path Length}

We test the RNN and GRU performance on a variety of Langevin systems with different memory properties. The results are shown in Fig.~\cref{fig:memory} (all are trained using Adam).
\begin{figure}[htb!]
    \centering
    \includegraphics[width=\textwidth]{figures/memory}
    \caption{Training (Adam) wrt memory.}
    \label{fig:memory}
\end{figure}


\newpage
\subsection{The Dynamics of the Gating Parameter}

Now, we investigate the dynamics of the gating parameters: $z_t$ (hidden gate) and $r_t$ (reset gate) in GRU as training proceeds, for a varieties of target dynamics. The observations are shown in Fig.~\cref{fig:gating}.
\begin{figure}[htb!]
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/gating_langevin.pdf}
        \caption{Langevin}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/gating_generalized_langevin_exp.pdf}
        \caption{Generalized Langevin (Exponential Kernel)}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/gating_generalized_langevin_powerlaw.pdf}
        \caption{Generalized Langevin (Power Law Kernel)}
    \end{subfigure}
    \caption{Dynamics of gating parameters.}
    \label{fig:gating}
\end{figure}


\begin{figure}
    \ContinuedFloat
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/gating_generalized_langevin_sine.pdf}
        \caption{Generalized Langevin (Sine Kernel)}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/gating_baseline.pdf}
        \caption{Baseline (Just some nonlinear function of the inputs, which is random noise)}
    \end{subfigure}
    \caption{Dynamics of gating parameters. The solution $\bs{y}_{0:T}$ (normalized to [0,1]) is overlaid for comparison of periodicity}
    \label{fig:gating}
\end{figure}

\newpage
\subsection{Summary of Findings and Next Steps}

Summary of Findings:
\begin{enumerate}
    \item Orthogonal initialization has marginally better performance (this is already noted in~\cite{saxeExactSolutionsNonlinear2014}) and is in fact the default init scheme in the new version of Keras/Tensorflow.
    \item Generally GRU is harder to train than RNN, but for larger time horizons $T$ performs better. In those cases, RNN training generally stalls.
    \item The explicit memory terms make RNN slightly harder to train. The point of the sine kernel is to show that this is an infinite memory kernel, but due to the averaging of the sine function, the effective path behaves much less erratic. However, the power-law kernel is a true long-memory kernel. In all cases, GRU performs better than RNN, especially for large $T$.
    \item On the dynamics of the gating parameters, it is observed that for memory systems and large time horizons, as training proceeds there tends to be oscillations in the gates. This is less pronounced in vanilla langevin and baseline systems.
\end{enumerate}

Next steps (theory)
\begin{enumerate}
    \item Come up with a strategy to investigate the above phenomenon mathematically.
    \item Relevant papers:~\cite{hardtGradientDescentLearns2019,millerStableRecurrentModels2019}
\end{enumerate}

Next steps (Experiments)
\begin{enumerate}
    \item Test the effect of $\gamma$ (implicit memory) on learning dynamics
    \item Variable time horizon (generalization, approximation and the like)
    \item Future: LSTM or transformer/attention networks~\cite{vaswaniAttentionAllYou2017}
\end{enumerate}

==> figures_fine_grain/conclusion.tex <==
\section{Conclusion}

In this paper, we analyzed the basic approximation and optimization aspects of using RNNs to learn input-output relationships involving temporal sequences in the linear, continuous-time setting.
% In both cases, our analysis reveals that the dynamical nature of the problem connects the idea of memory and learning in a precise way. 
In particular, we coined the concept \emph{curse of memory}, and revealed two of its facets. That is, when the target relationship has the long term memory, both approximation and optimization become exceedingly difficult. These analyses make concrete heuristic observations of the adverse effect of memory on learning RNNs. Moreover, it quantifies the interaction between the structure of the model (RNN functionals) and the structure of the data (target functionals). The latter is a much less studied topic.
Here, we adopt a continuous-time approach in order gain access to more quantitative tools, including classical results in approximation theory and stochastic analysis, which help us derive precise results in approximation rates and optimization dynamics. The extension of these results to discrete time may be performed via numerical analysis in subsequent work.
More broadly, this approach may be a basic starting point for understanding learning from partially observed time series data in general, including gated RNN variants \citep{hochreiter1997long,cho2014} and other methods such as transformers and convolution-based approaches \citep{vaswani2017attention,oord2016wavenet}. These are certainly worthy of future exploration.

==> formulation.tex <==
\subsection{Problem Formulation}

We will proceed as in supervised learning, but with inputs and outputs as time series data.

\paragraph{Input and Output Spaces.}
Let the input space be the space of continuous functions from $\R$ (time) to $\R^d$ that vanishes at infinity:
%\JH{Do we only need it vanishes at $-\infty$ and bounded on $\R$?}
\begin{align}
    \Xcal = C_0(\R, \R^d).
    % \left\{
    %     \bs{x} \in C_0(\R, \R^d):
    %     \sup_{t\neq s} \frac{\|x_t - x_s\|_\infty}{|t-s|^{\gamma}} < \infty
    % \right\}
\end{align}
For the space of outputs we will take a scalar time series, i.e. the space of bounded continuous functions from $\R$ to $\R$:
\begin{align}
    \Ycal =
    C_b(\R, \R).
\end{align}
We will equip $\Xcal$ with the supremum norm
\begin{align}
    \| \bs{x} \|_\Xcal \coloneqq \sup_{t \in \R} \| x_t \|_\infty.
    % = \sup_{t \in \R} \max_{i=1,\dots,d} | x_{t, i} |.
    % + \sup_{t\n0eq s} \frac{\|x_t - x_s\|_\infty}{|t-s|^{\gamma}}
\end{align}
% where $\|\cdot \|$ is the usual Euclidean norm on $\R^d$.

% \begin{align}
%     \{ x_t \in \R^d : -\infty < t < \infty \}
%     \qquad \text{and} \qquad
%     \{ y_t \in \R : -\infty < t < \infty \}
% \end{align}
% representing the inputs and outputs. We will assume that $x_t$ is continuous and bounded for $t\in \R$ with $\sup_{s\in\R}|x_s| = M$

\paragraph{Notation for Paths.}
Let us also define the shorthand $\bs{x}_{s:t} := \{ x_{r} : r\in[s, t] \}$. Similarly, we write $\bs{x}_{:s} := \{x_{r} : -\infty < r \leq s\}$ and similarly for $\bs{x}_{s:}$. Finally we write $\bs{x} := \{x_r: r\in \R\} \in \Xcal$. Similar notation will be used for $\bs{y} \in \Ycal$.

\paragraph{Ground Truth or Oracle.}
We now assume an underlying ground truth relationship between inputs $\bs{x}$ and outputs $\bs{y}$ as follows:
\begin{align}
    y_t = H_{t}(\bs{x}),
\end{align}
where for each $t\in\R$, $H_{t}$ is a functional
\begin{align}
    H_{t} : \Xcal \rightarrow \R.
\end{align}
Let us assume for the moment that the family of functionals $\{ H_t : t\in\R \}$ satisfies the continuity condition
\begin{align}
    \lim_{\delta \rightarrow 0} H_{t+\delta} (\bs{x}) = H_{t} (\bs{x})
    \qquad
    \text{for all } t\in\R, \bs{x}\in\Xcal.
\end{align}
This ensures that $y_t = H_t(\bs{x})$ is continuous in $t$. Later we will show that this is a consequence of other restrictions we may wish to place on the family.

\paragraph{Some Types of Functionals.}

Here, we define some specific types of functionals we may be interested in.

\begin{definition}[Causal Functionals]
    We call $H_t$ a causal functional if it does not depend on the future values of $\bs{x}_{t:}$. Concretely, for each $t\in \R$, if $\bs{x},\bs{x'} \in \Xcal$ are such that
    \begin{align}
        x_{s} = x'_{s} \text{ for all } s \leq t,
    \end{align}
    then we have $H_t(\bs{x}) = H_t(\bs{x'})$.
\end{definition}

\begin{definition}[Continuous Linear Functionals]
    We call $H$ a continuous linear functional if for any $\bs{x},\bs{x'} \in \Xcal$ and $\lambda,\lambda'\in \R$ we have
    \begin{align}
        H(\lambda \bs{x} + \lambda' \bs{x'})
        = \lambda H(\bs{x}) + \lambda' H(\bs{x'})
    \end{align}
    and moreover that
    \begin{align}
        \sup_{\bs{x} \in \Xcal, \| \bs{x} \|_\Xcal \leq 1} H(\bs{x}) < \infty,
    \end{align}
    in which case we can define the induced norm on the dual space of $\Xcal$ as
    \begin{align}
        \| H \| \coloneqq \sup_{\bs{x} \in \Xcal, \| \bs{x} \|_\Xcal \leq 1} | H(\bs{x}) |,
        \qquad
        H \in \Xcal^*.
    \end{align}
    We say that a family $\{H_t\}$ is continuous and linear if each $H_t$ is continuous and linear.
\end{definition}

\begin{definition}[Regular Functionals]
    We say that a functional $H : \Xcal \rightarrow \R$ is regular if for any sequence $\{\bs{x}^{(n)} \in \Xcal, : n \geq 0\}$ such that $x_t^{(n)} \rightarrow 0$ for almost every $t\in\R$ (in the sense of Lebesgue measure), then
    \begin{align}
        \lim_{n\rightarrow \infty} H(\bs{x}_n) = 0.
    \end{align}
    We say that the family $\{H_t\}$ is regular if each $H_t$ is regular.
\end{definition}

\begin{definition}[Time Homogeneous Functionals]
    We say a family of functionals $\{ H_{t} : t \in \R \}$ is \emph{time homogeneous} if for every $t,\tau\in \R$, we have
    \begin{align}\label{eq:defn_time_homo}
        H_{t}(\bs{x}) = H_{t+\tau}(\bs{x}^{(\tau)})
    \end{align}
    where $x^{(\tau)}_s = x_{s - \tau}$ for all $s$, i.e. $\bs{x}^{(\tau)}$ is $\bs{x}$ shifted by $\tau$.
\end{definition}

\paragraph{Recurrent Neural Nets.}
Recurrent neural networks can be seen as a way to model this functional, in the form of a hidden dynamics:
\begin{align}\label{eq:hidden_dyn}
    \begin{split}
        \wh{y}_t &= g_\phi(h_t), \\
        \frac{dh_t}{dt} &= f_\theta(h_t, x_t),
    \end{split}
\end{align}
where each $h_t \in \R^m$ denotes a hidden (latent) state with dimension $m$. The functions
$g_\phi : \R^m \rightarrow \R$ and $f_\theta : \R^m \times \R^d \rightarrow \R^m$ are taken from some parametric family $\Fcal$ and $\Gcal$ respectively:
\begin{align}
    \Fcal = \{f_\theta : \theta\in\Theta\},
    \qquad
    \Gcal = \{g_\phi : \phi\in\Phi\}.
\end{align}

==> gating.tex <==
\section{Gating Mechanism}

It is of interest to ask what happens when a gate is applied to the RNN hidden dynamics as follows
\begin{align}\label{eq:rnn_gate}
    \begin{split}
        &\dot{h}_t = W h_t \circ r_t + b x_t \\
        &r_t = \sigma(W_r h_t + b_r x_t + \xi)
    \end{split}
\end{align}
where $W_r \in \R^{m\times m}, b_r \in \R^m, \xi \in \R$. The variable $r_t$ is known as a \emph{reset gate} commonly applied to GRU/LSTM-type architectures. It is our goal to investigate its effect on the network in terms of approximation and optimization.

Although~\cref{eq:rnn_gate} cannot be solved explicitly, we can nevertheless make some observations. First, by setting $W_r = b_r = 0$ and $\xi \rightarrow \infty$ we can recover the usual RNN, so from an approximation point of view the space of linear functionals that can be approximated is at least as large as in the usual RNN case. Moreover, we can write the output corresponding to~\cref{eq:rnn_gate} as
\begin{align}
    \begin{split}
        &\wh{w}_t = \int_{0}^{t} c^\tp e^{W R_s} b x_{t-s} ds, \\
        &R_t =  \mathrm{diag}
        \left[
            \int_{0}^{t} \sigma(W_r h_s + b_r x_s + \xi) ds.
        \right]
    \end{split}
\end{align}
When used to approximate a linear functional, the only difference now is that, instead of approximating the measure $\rho(s)$ by the exponential sum $c^\tp e^{W s} b$, we now approximate the measure by $c^\tp e^{W R_s} b$. But, element-wise $0 < R_s < s$ for all $s$ and $R_s$ is strictly increasing in $s$, hence it gives in effect another ``parameterization'' of time. In particular, it is plausible that $c^\tp e^{W R_s} b$ can approximate a non-exponential-decaying $\rho(s)$. We know that in the case of linear RNN corresponding to approximating $\rho(s)$ by exponential sums, it is necessary that $\rho(s)$ decreases exponentially for approximation to hold on $t\in[0,\infty)$.

\recheck{How do we show this more precisely in a mathematical sense?}

==> nonlinear.tex <==
\section{Nonlinear Extension, Monte-Carlo (Barron Space) Interpretation}

==> outline.tex <==
\section*{Paper Outline}

\hl{Highlighted text is TODO} 

\begin{enumerate}
    \item Introduction and Motivation
    \begin{enumerate}
        \item The need for a similar theory to supervised learning of functions, but with temporal dynamics and functionals as target objects
        \item The need to understand why RNNs are hard to train, and how to overcome it
    \end{enumerate}
    \item An Approximation Theory for RNNs
    \begin{enumerate}
        \item Universal approximation of linear functionals in 1D (1 dim time series) by linear RNNs
        \item \hl{Universal approximation in higher dimensions and overcome curse of dimensionality}
    \end{enumerate}
    \item Understanding The Difficulty of RNN Training
    \begin{enumerate}
        \item Experimental phenomenon of plateauing
        \item Symmetry argument and asymptotic analysis for 2 dimensional case
        \item \hl{Curse of dimensionality of asymptotics for higher dimensional case}
    \end{enumerate}
    \item \hl{Algorithm to Improve Performance}
\end{enumerate}


==> preamble.tex <==
% General document formatting
\usepackage[margin=0.7in]{geometry}
\usepackage[parfill]{parskip}
\usepackage[utf8]{inputenc}
\usepackage[tt=false, type1=true]{libertine}
\usepackage[varqu]{zi4}
\usepackage{color}
\usepackage{subcaption}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{bbm}
\usepackage{bm}
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{caption}
\usepackage{verbatim}
\usepackage{authblk}


==> rnn_variants.tex <==
\section{Variants of RNNs}

We will now work in discrete time to conform with notation in machine learning. Here we consider a few variants of RNNs:

\begin{enumerate}
    \item Vanilla Recurrent Neural Networks
    \begin{align}
        \begin{split}
            h_t &= \sigma_h(W_h x_t + U_h h_{t-1} + b_h)
        \end{split}
    \end{align}
    \item Gated Recurrent Units (See also variants in~\cite{deyGateVariantsGatedRecurrent})
    \begin{align}
        \begin{split}
            z_{t}&=\sigma_{g}\left(W_z x_{t} + U_z h_{t-1} + b_z \right) \\
            r_{t}&=\sigma_{g}\left(W_r x_{t} + U_r h_{t-1} + b_r \right) \\
            h_{t}
            &=
            z_{t}
            \circ h_{t-1} + (1 - z_{t}) \circ
            \sigma_h
            \left(
                W_{h} x_{t} + U_{h} (r_{t} \circ h_{t-1} ) + b_h
            \right)
            ,\qquad h_0 = 0
        \end{split}
    \end{align}
    \item Long Short Term Memory (See also variants in \url{https://en.wikipedia.org/wiki/Long_short-term_memory})
    \begin{align}
        \begin{split}
            f_{t}&=\sigma_{g}\left(W_f x_{t} + U_f h_{t-1} + b_f \right) \\
            i_{t}&=\sigma_{g}\left(W_i x_{t} + U_i h_{t-1} + b_i \right) \\
            o_{t}&=\sigma_{g}\left(W_o x_{t} + U_o h_{t-1} + b_o \right) \\
            c_{t}
            &=
            f_t \circ c_{t-1}
            + i_t \circ \sigma_c(W_c x_t + U_c h_{t-1} + b_c) \\
            h_t &= o_t \circ \sigma_h(c_t)
            ,\qquad h_0 = c_0 = 0
        \end{split}
    \end{align}
\end{enumerate}
